iFlame: Interleaving Full and Linear Attention for Efficient Mesh Generation

This paper propose iFlame, a novel transformer-based network architecture for mesh generation. While attention-based models have demonstrated remarkable performance in mesh generation, their quadratic computational complexity limits scalability, particularly for high-resolution 3D data. Conversely, linear attention mechanisms offer lower computational costs but often struggle to capture long-range dependencies, resulting in suboptimal outcomes. To address this trade-off, we propose an interleaving autoregressive mesh generation framework that combines the efficiency of linear attention with the expressive power of full attention mechanisms. To further enhance efficiency and leverage the inherent structure of mesh representations, we integrate this interleaving approach into an hourglass architecture, which significantly boosts efficiency. Our approach reduces training time while achieving performance comparable to pure attention-based models. To improve inference efficiency, we implemented a caching algorithm that almost doubles the speed and reduces the KV cache size by seven-eighths compared to the original Transformer. We evaluate our framework on ShapeNet and Objaverse, demonstrating its ability to generate high-quality 3D meshes efficiently. Our results indicate that the proposed interleaving framework effectively balances computational efficiency and generative performance, making it a practical solution for mesh generation. The training takes only 2 days with 4 GPUs on 39k data with a maximum of 4k faces on Objaverse.

==> tikz_fig/performance_backup.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{0.23\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width=5pt,
    ylabel={Throughput (t/s)},
    symbolic x coords={Minimax,Linear,Standard,Ours},
    xtick=data,
    xticklabels={Minimax,Linear att.,Standard att.,Ours},
    x tick label style={
        font=\footnotesize,
        rotate=45,
        anchor=east
    },
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={font=\footnotesize},
    ymin=0,
    ymax=100,
    enlarge x limits=0.25,
    ylabel near ticks,
    ylabel style={
        font=\footnotesize,
        rotate=0
    },
    y tick label style={
        font=\footnotesize,
        rotate=90
    },
    title={Inference Throughput},
    title style={font=\footnotesize},
]
\addplot[fill=gray!50] coordinates {
    (Minimax, 38.9)
    (Linear, 40.8)
    (Standard, 45.0)
    (Ours, 81.9)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hspace{-3em}
\hfill
\begin{subfigure}{0.23\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width=5pt,
    ylabel={KV Cache (GB)},
    symbolic x coords={Minimax,Linear,Standard,Ours},
    xtick=data,
    xticklabels={Minimax,Linear att.,Standard att.,Ours},
    x tick label style={
        font=\footnotesize,
        rotate=45,
        anchor=east
    },
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={font=\footnotesize},
    ymin=0,
    ymax=8,
    enlarge x limits=0.25,
    ylabel near ticks,
    ylabel style={
        font=\footnotesize,
        rotate=0
    },
    y tick label style={
        font=\footnotesize,
        rotate=90
    },
    title={Memory Efficiency},
    title style={font=\footnotesize},
]
\addplot[fill=gray!50] coordinates {
    (Minimax, 0.8)
    (Linear, 0.0)
    (Standard, 6.6)
    (Ours, 0.8)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hspace{-3em}
\hfill
\begin{subfigure}{0.23\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width=5pt,
    ylabel={Time (min)},
    symbolic x coords={Minimax,Linear,Standard,Ours},
    xtick=data,
    xticklabels={Minimax,Linear att.,Standard att.,Ours},
    x tick label style={
        font=\footnotesize,
        rotate=45,
        anchor=east
    },
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={font=\footnotesize},
    ymin=0,
    ymax=500,
    enlarge x limits=0.25,
    ylabel near ticks,
    ylabel style={
        font=\footnotesize,
        rotate=0
    },
    y tick label style={
        font=\footnotesize,
        rotate=90
    },
    title={Training Time},
    title style={font=\footnotesize},
]
\addplot[fill=gray!50] coordinates {
    (Minimax, 341)
    (Linear, 304)
    (Standard, 422)
    (Ours, 227)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hspace{-3em}
\hfill
\begin{subfigure}{0.23\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width=5pt,
    ylabel={Memory (GB)},
    symbolic x coords={Minimax,Linear,Standard,Ours},
    xtick=data,
    xticklabels={Minimax,Linear att.,Standard att.,Ours},
    x tick label style={
        font=\footnotesize,
        rotate=45,
        anchor=east
    },
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={font=\footnotesize},
    ymin=0,
    ymax=80,
    enlarge x limits=0.25,
    ylabel near ticks,
    ylabel style={
        font=\footnotesize,
        rotate=0
    },
    y tick label style={
        font=\footnotesize,
        rotate=90
    },
    title={Training Memory},
    title style={font=\footnotesize},
]
\addplot[fill=gray!50] coordinates {
    (Minimax, 63)
    (Linear, 50)
    (Standard, 45)
    (Ours, 28)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hspace{-3em}
\hfill
\begin{subfigure}{0.23\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width=5pt,
    ylabel={Face Accuracy},
    symbolic x coords={Minimax,Linear,Standard,Ours},
    xtick=data,
    xticklabels={Minimax,Linear att.,Standard att.,Ours},
    x tick label style={
        font=\footnotesize,
        rotate=45,
        anchor=east
    },
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={font=\footnotesize},
    ymin=70,
    ymax=80,
    enlarge x limits=0.25,
    ylabel near ticks,
    ylabel style={
        font=\footnotesize,
        rotate=0
    },
    y tick label style={
        font=\footnotesize,
        rotate=90
    },
    title={Model Perplexity},
    title style={font=\footnotesize},
]
\addplot[fill=gray!50] coordinates {
    (Minimax, 77.8)
    (Linear, 71.9)
    (Standard, 78.3)
    (Ours, 78.1)
};
\end{axis}
\end{tikzpicture}
\end{subfigure}

\caption{Performance comparison of our alternating hourglass architecture. \textbf{(a)} Our model achieves 1.8$\times$ higher inference throughput (81.9 t/s vs. 45.0 t/s). \textbf{(b)} Our model maintains low KV cache usage (0.8GB) while standard attention requires 8.3$\times$ more memory. \textbf{(c)} Our model reduces training time by 46\% (227 min vs. 422 min). \textbf{(d)} Our model requires 38\% less GPU memory during training (28GB vs. 45GB per GPU). \textbf{(e)} Our model maintains face accuracy (78.1\% vs. 78.3\%) compared to baseline methods.}
\label{fig:performance_comparison}
\end{figure*}
